Reinforcing Adversarial Robustness using Model Confidence Induced by Adversarial Training

In this paper we study leveraging confidence information induced by adversarial training to reinforce adversarial robustness of a given adversarially trained model. A natural measure of confidence is $\|F({\bf x})\|_\infty$ (i.e. how confident $F$ is about its prediction?). We start by analyzing an adversarial training formulation proposed by Madry et al.. We demonstrate that, under a variety of instantiations, an only somewhat good solution to their objective induces confidence to be a discriminator, which can distinguish between right and wrong model predictions in a neighborhood of a point sampled from the underlying distribution. Based on this, we propose Highly Confident Near Neighbor (${\tt HCNN}$), a framework that combines confidence information and nearest neighbor search, to reinforce adversarial robustness of a base model. We give algorithms in this framework and perform a detailed empirical study. We report encouraging experimental results that support our analysis, and also discuss problems we observed with existing adversarial training.

==> Makefile <==
### Makefile --- 

TARGETS = paper

%: %.tex
	latexmk -g -pdf -silent $@ # generate pdf
	latexmk -c $@ # clean up regeneratable files

all: pdf

pdf: ${TARGETS}

clean:
	@echo cleaning up...
	rm -f *.fdb_latexmk *.ps *.dvi *.aux *.bbl *.blg *.brf *.cb *.cb2 \
		 *.idx *.ilg *.ind *.inx *.log *.mpx *.toc *.out *.pstex_t \
		 *.fig.bak  *.ps_e *~ *.tex.* *.thm *.fls



==> discussion.tex <==
We now discuss our method and results.

\noindent\textbf{Our technical contributions.}
Our first technical contribution is the proposal to take into account the inherent confidence information
produced by models when studying adversarial perturbations.
Our second technical contribution is a formulation of a goodness property of models,
and an analysis of existing models in view of the property. Interestingly, and somewhat surprisingly,
we find that a recent robust training objective function by~\cite{MMSTV17} encourages good separation of
high-confidence points, but has essentially no control of low-confidence points.
Our third contribution is the proposal of embedding to handle low-confidence points.
Our final contribution is a first empirical study that validates Madry et al.'s model
in terms of the goodness property, and further demonstrates that a good model, when wrapped with embedding,
simultaneously achieves good generalization and almost perfect robustness.

\noindent\textbf{Interpretations of our results.}
One interpretation of our results is that adversarial perturbations can
\emph{naturally coexist with good generalization}.
While this is manifested in our analysis of Madry et al.'s objective function,
we think that this phenomenon naturally and generally exists if one takes again a manifold point of view:
Since natural manifolds reside in low dimensions, it seems much more challenging to control the confidence
boundary, where ``adversarial perturbations'' exist in abundance, than controlling separation of
the learned structures (i.e. confident regions that approximate the underlying manifolds).

On the other hand, if all one cares about is robustness (decision does not change in a small neighborhood),
then adversarial perturbation problem can be resolved by combining goodness property with embedding.
For example, consider the following ``good model:'' If a data point is from the training set,
then it outputs the correct label with confidence $1$, otherwise it outputs a uniform distribution over labels.
In other words, this model learns nothing but fitting the training set.
We note that in this case, the adversarial perturbation problem is \emph{only well defined}
around the training points.
Moreover, embedding now becomes $1$-nearest neighbor search among the training points.
As a result, the model is still \emph{perfectly robust} with our method if training points are well separated.

\noindent\textbf{Highly confident predictions on random noises.}
We note that several work shows that neural networks can have highly confident predictions on random noises
(e.g.,~\cite{NYC15}). In view of our work it is somewhat not surprising that neural networks can have such behaviors:
These points are essentially ones that are \emph{far away from} the ``universe'' the learner is asked to learn,
and so if we do not control the training of neural networks to not claim confidence over the structure
it has never seen, then it is valid to fit a model that has good behaviors on natural manifolds
but also divergent behaviors outside. After all, why is a network supposed to work on points that are far away
from the underlying natural manifolds, which is essentially the \emph{data generating distribution?}
Finally, we note that the adversarial perturbation problem is not well defined even near those points.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "make"
%%% End: 

